SEED: Self-supervised Distillation For Visual Representation

This paper is concerned with self-supervised learning for small models. The problem is motivated by our empirical studies that while the widely used contrastive self-supervised learning method has shown great progress on large model training, it does not work well for small models. To address this problem, we propose a new learning paradigm, named SElf-SupErvised Distillation (SEED), where we leverage a larger network (as Teacher) to transfer its representational knowledge into a smaller architecture (as Student) in a self-supervised fashion. Instead of directly learning from unlabeled data, we train a student encoder to mimic the similarity score distribution inferred by a teacher over a set of instances. We show that SEED dramatically boosts the performance of small networks on downstream tasks. Compared with self-supervised baselines, SEED improves the top-1 accuracy from 42.2% to 67.6% on EfficientNet-B0 and from 36.3% to 68.2% on MobileNet-v3-Large on the ImageNet-1k dataset.

==> ICLR20_Distillatio (2)/abstract.tex <==
\vspace{-2mm}
\begin{abstract}
% With the rapid development of contrastive self-supervised learning, works sprang out till now are unanimously laid upon the objective of higher accuracy with larger deep networks. Hereby, we further study this from the perspective of \textbf{SE}lf-Sup\textbf{E}rvised \textbf{D}istillation ({\large S}EED) as a new learning paradigm,  where we leverage larger networks (as Teacher) to transfer representational knowledge with stronger discrimination into smaller architectures (as Student) in the setting of self-supervised learning.  
% Instead of directly learn from the unlabeled data, we simply train the student encoder to mimic the similarity score distribution over a set of instances with the teacher.
% Instead of directly learning from unlabeled data, we train the student so that it is similar to the teacher for both the augmented view of a positive instance and the randomly-sampled negative samples
% We show that with {\large S}EED, it dramatically boosts the performances of the shallow networks on downstream tasks with the distillation from a self-supervised pre-trained cumbersome network. Comparing with self-supervised baseline, {\large S}EED improves the top-1 accuracy of efficientNet-b0 from 42.2\% to 65.3\% and from 36.3\% to 61.4\% on MobileNet-v3-large with only 5M parameters on ImageNet-1k Dataset.  We also show that {\large S}EED consistently outperforms unsupervised contrastive baseline models on various architectures, providing cogent and detailed guidance for practitioners to acquire smaller yet stronger models easily in unsupervised scenarios.  
This paper is concerned with self-supervised learning for small models. The problem is motivated by our empirical studies that while the widely used contrastive self-supervised learning method has shown great progress on large model training, it does not work well for small models. To address this problem, we propose a new learning paradigm, named \textbf{SE}lf-Sup\textbf{E}rvised \textbf{D}istillation ({\large S}EED), where we leverage a larger network (as Teacher) to transfer its representational knowledge into a smaller architecture (as Student) in a self-supervised fashion. Instead of directly learning from unlabeled data, we train a student encoder to mimic the similarity score distribution inferred by a teacher over a set of instances. We show that {\large S}EED dramatically boosts the performance of small networks on downstream tasks. Compared with self-supervised baselines, {\large S}EED improves the top-1 accuracy from 42.2\% to 67.6\% on EfficientNet-B0 and from 36.3\% to 68.2\% on MobileNet-V3-Large on the ImageNet-1k dataset. 

% Recently there has been a lot of progress on self-supervised learning where much of the focus is on large models, but little attention has been paid to small models. In fact, as we will show in the paper, the commonly used contrastive self-supervised learning method does not work well for small models. To address this problem, we propose a new learning paradigm, named \textbf{SE}lf-Sup\textbf{E}rvised \textbf{D}istillation ({\large S}EED), where we leverage larger networks (as Teacher) to transfer  its representational knowledge into smaller architectures (as Student) in a self-supervised fashion. Instead of directly learn from the unlabeled data, we train the student encoder to mimic the similarity score distribution over a set of instances with the teacher. We show that {\large S}EED dramatically boosts the performance of small networks on downstream tasks. Compared with self-supervised baseline, {\large S}EED improves the top-1 accuracy of efficientNet-b0 from 42.2\% to 65.3\% and from 36.3\% to 61.4\% on MobileNet-v3-large with only 5M parameters on ImageNet-1k Dataset.  We also show that {\large S}EED consistently outperforms state-of-the-art unsupervised contrastive baseline models.
\end{abstract}
\vspace{-2mm}


==> ICLR20_Distillatio (2)/command.tex <==

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\xpar}[1]{\noindent\textbf{#1}\ \ }
\newcommand{\vpar}[1]{\vspace{3mm}\noindent\textbf{#1}\ \ }

\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\ssect}[1]{\S~\ref{#1}}
\newcommand{\eqn}[1]{Equation~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\tbl}[1]{Table~\ref{#1}}

\newcommand{\shapenet}{ShapeNet\xspace}
\newcommand{\pascal}{PASCAL 3D+\xspace}

\newcommand{\degree}{\ensuremath{^\circ}\xspace}
\newcommand{\ignore}[1]{}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\fcseven}{$\mbox{fc}_7$}

\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

\def\naive{na\"{\i}ve\xspace}
\def\Naive{Na\"{\i}ve\xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}

\newcommand{\yl}[1]{\textcolor{MyRed}{[Yonglong: #1]}}


\def\bR{\mathbb{R}}
\def\cL{\mathcal{L}}

\newcommand{\myparagraph}[1]{\vspace{-10pt}\paragraph{#1}}
\newcommand{\myitem}{\vspace{-5pt}\item}


\newcommand{\methodname}{dense convolutional  network}
\newcommand{\methodnamecap}{Dense Convolutional Network}
\newcommand{\methodnameshort}{DenseNet}
\newcommand{\methodnameshorts}{DenseNets}
\newcommand{\methodblock}{dense block}
\newcommand{\methodblockcap}{Dense Block}

\newcommand{\regmethodname}{feature drop}
\newcommand{\regmethodnamecap}{Feature Drop}

\newcommand{\stepsizename}{growth rate}

\newcommand{\conv}[1]{$\left[\begin{array}{ll} \text{1}\times \text{1} \text{ conv}\\ \text{3}\times \text{3} \text{ conv} \end{array}\right] \times \text{#1}$}

\newcommand{\bsk}[1]{$\text{Basic Block} \times \text{#1}$}
\newcommand{\bnk}[1]{$\text{Bottleneck Block} \times \text{#1}$}

\newcommand{\cross}[1]{#1 $\times$ #1}

\newcommand{\feati}{x_i}
\newcommand{\clsfeati}{y_i}
\newcommand{\featk}{x_k}
\newcommand{\clsfeatk}{y_k}
\newcommand{\loss}{L}
\newcommand{\featL}{x_L}
\newcommand{\clsfeat}{y}
\newcommand{\anyxs}{\ensuremath{\mathbf{x}}}
\newcommand{\anyys}{\ensuremath{\mathbf{y}}}

\newcommand{\bx}{\ensuremath{\mathbf{x}}}

\newcommand{\sourcexs}{\ensuremath{\mathbf{x^\mathcal{S}}}}
\newcommand{\sourceys}{\ensuremath{\mathbf{y^\mathcal{S}}}}

\newcommand{\targetxs}{\ensuremath{\mathbf{x^\mathcal{T}}}}
\newcommand{\targetys}{\ensuremath{\mathbf{y^\mathcal{T}}}}
\newcommand{\pseudotargetys}{\ensuremath{\mathbf{\hat{y}^\mathcal{T}}}}


% \newcommand*{\thead}[1]{\multicolumn{1}{c}{\begin{tabular}{@{}c@{}}#1\end{tabular}}}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand*{\mathcolor}{}
\def\mathcolor#1#{\mathcoloraux{#1}}
\newcommand*{\mathcoloraux}[3]{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}

\definecolor{darkgreen}{RGB}{0,112,0}


==> ICLR20_Distillatio (2)/experiment.tex <==

\section{Experiment}
\label{sec:exp}
\subsection{Pre-training}

\noindent \textbf{Self-Supervised Pre-training of Teacher Network.} \; 
% We use the adapted version of MoCo~\citep{chen2020improved}, MoCo-V2, as our self-supervised pre-training method for the pre-training of teacher architecture. We also show results with several other self-supervised pre-trained models as the teacher of distillation in ablations, which yield similar conclusions. Following~\citep{chen2020simple}, we use ResNet as the network architecture with different depths/widths (\textit{e.g.}, 50, 101 and 152 layers and $\times$1, $\times$2 parameters in ResBlock). MoCo-V2 has a multi-layer-perception (MLP) layer at the end of the encoder after average pooling, which contains two linear layers and one \textit{ReLU}~\citep{nair2010rectified} activation layer. We use the produced 128d vector from \textit{MLP} as our image representation $\mathbf{z}$ for both pre-training and distillation. All teacher networks are pre-trained for 200 epochs with a queue of 65,356 data samples on the {ImageNet ILSVRC-2012} dataset~\citep{deng2009imagenet}. Due to the computational limit, we pre-train our teacher network as well as the distillation process for 200 epochs unless explicitly note.
By default, we use MoCo-V2~\citep{chen2020improved}
to pre-train the teacher network.
Following~\citep{chen2020simple}, we use ResNet as the network backbone with different depths/widths and append a multi-layer-perceptron (MLP) layer (two linear layers and one \textit{ReLU}~\citep{nair2010rectified} activation layer in between) at the end of the encoder after average pooling. 
The dimension of the last feature dimension is 128. All teacher networks are pre-trained for 200 epochs due to the computational limitation unless explicitly specified.
As our distillation is independent with the teacher pre-training algorithm, we also show results with  other self-supervised pre-trained models for teacher network, \textit{e.g.}, {\large S}WAV~\citep{caron2020unsupervised}, SimCLR~\citep{chen2020simple}.




\noindent \textbf{Self-Supervised Distillation on Student Network.}
\; We choose multiple smaller networks with fewer learnable parameters as the student network: MobileNet-v3-Large~\citep{howard2017mobilenets}, EfficientNet-B0~\citep{tan2019efficientnet}, and smaller ResNet with fewer layers (ResNet-18, 34). Similar to the pre-training for teacher network, we add one additional MLP layer on the basis of the student network.  Our distillation is trained with a standard SGD optimizer with momentum 0.9 and a weight decay parameter of 1e-4 for 200 epochs.  The initial learning rate is set as 0.03 and updated by a cosine decay scheduler~\citep{nair2010rectified} with 5 warm-up epochs and batch size 256.
% We linearly scale the base learning rate (LR) with the batch size (BS) increase, that is, LR = 0.03 $\times$BS/256~\citep{goyal2017accurate}. 
In \textit{Eq.}~\ref{eq:finalloss}, the teacher temperature is set as $\tau^T=0.01$ and the student temperature is $\tau^S=0.2$. The queue size of $K$ is 65,536.
%In terms of the training cost, it takes approximately 40 hours for the distillation of EfficientNet-B0 from ResNet-50 with 8$\times$NVIDIA V100 GPUs on ImageNet without any special accelerating measure. 
In the following subsections and appendix, we also show results with different hyper-parameter values, \textit{e.g.}, for $\tau^T$ and $K$.


% \; In order to compare the effect of distillation on various networks, we chose multiple smaller networks with fewer learnable parameters as the distillation target: MobileNet-v3-Large~\citep{howard2017mobilenets}, EfficientNet-B0~\citep{tan2019efficientnet}, and smaller residual neural networks with fewer layers (ResNet-18, 34). Similar to MoCo-V2, we add one additional linear layer in the last MLP block on the basis of primitive design of EfficientNet and MobileNet. We use a standard SGD optimizer with momentum 0.9 and a weight decay parameter of 1e-4 for 200 epochs. The initial learning rate is set as 0.03 and updated by a cosine decay scheduler~\citep{loshchilov2016sgdr} with 5 warm-up epochs and batch size to be 256. We linearly scale the base learning rate (LR) with the batch size (BS) increase, that is, LR = 0.03 $\times$BS/256~\citep{goyal2017accurate}. The teacher temperature is set at a smaller value $\tau^T=0.01$ than the student temperature, $\tau^S=0.2$. During the distillation, we maintain a standard queue with the length to be 65,536 as in MoCo. In terms of the training cost, it takes approximately 40 hours for the distillation of EfficientNet-B0 from ResNet-50 with 8$\times$NVIDIA V100 GPUs on ImageNet without any special accelerating measure. We further discuss effect of different hyper-parameters in ablations.


% \subsection{Scheme for Validity}
\subsection{Fine-tuning and evaluation}
In order to validate the effectiveness of self-supervised distillation, we choose to assess the performance of representations of the student encoder on several downstream tasks. We first report its performances of linear evaluation and semi-supervised linear evaluation on the ImageNet ILSVRC-2012~\citep{deng2009imagenet} dataset. To measure the feature transferability brought by distillation, we also conduct evaluations on other tasks, which include object detection and segmentation on the VOC07~\citep{pascal-voc-2007} and MS-COCO~\citep{lin2014microsoft} datasets. At the end, we compare the transferability of the features learned by distillation with ordinary self-supervised contrastive learning on the tasks of linear classification on datasets from different domains.


\noindent \textbf{Linear and \textit{K}NN Evaluation on ImageNet.}  \;
We conduct the supervised linear classification on ImageNet-1K, which contains $\sim$1.3M images for training, and 50,000 images for validation, spanning 1,000 categories. Following previous works in~\citep{he2020momentum,chen2020simple}, we train a single linear layer classifier on top of the frozen network encoder after self-supervised pre-training/distillation. SGD optimizer is used to train the linear classifier for 100 epochs with weight decay to be 0. The initial learning rate is set as 30 and is then reduced by a factor of 10 at 60 and 80 epochs (similar as in ~\cite{tian2019contrastive}). Notably, when training the linear classifier for MobileNet and EfficientNet, we reduce the initial learning rate to 3. The results are reported in terms of Top-1 and Top-5 accuracy. We also perform classification using \textit{K}-Nearest Neighbors (\textit{K}NN) based on the learned 128d vector from the last MLP layer. The sample is classified by taking the most frequent label of its $K$ ($K=10$) nearest neighbors.

Table~\ref{tbl:imgnet} shows the results with various teacher networks and student networks. We list the baseline of contrastive self-supervised pre-training using MoCo-V2~\citep{chen2020improved} in the first row for each student architecture. We can see clearly that smaller networks perform rather worse. For example, MobileNet-V3 can only reach 36.3\%. This aligns well with previous conclusions from~\citep{chen2020simple,chen2020big} that bigger models are desired to perform better in contrastive-based self-supervised pre-training. We conjecture that this is mainly caused by the inability of smaller network to discriminate instances in a large-scale dataset.
The results also clearly demonstrate that the distillation from a larger network helps boosting the performances of small networks, and show obvious improvement.
%compared with the ordinary contrastive self-supervised pre-training.
For instance, with MoCo-V2 pre-trained ResNet-152 (for 400 epochs) as the teacher network, the Top-1 accuracy of MobileNet-V3-Large can be significantly improved from 36.3\% to 61.4\%.
% outperforming ResNet-34 (4$\times$larger than EfficientNet-B0) trained using MoCo-V2 without distillation by a large margin of 8.0\%, and even approaching the performances of MoCo-V2 using ResNet-50 on the linear evaluation task. 
Furthermore, we
use ResNet-50${\times2}$ (provided in~\cite{caron2020unsupervised}) as the teacher network and adopt the multi-crop trick (see~\ref{sup:eval} for details). 
The accuracy can be further improved to 68.2\% (last row of Table~\ref{tbl:imgnet}) for MobileNet-V3-Large with 800 epochs of distillation. We note that the gain benefited from distillation becomes more distinct on smaller architectures and we further study the effect of various teacher models in ablations.
\input{tables/distill_imgnet}

% To test the distillation effect on larger student encoders, we also report the distillation results using ResNet-50 (see Appendix), and observe the same improvement trend: it reaches 74.3\%  Top-1 accuracy with  ResNet-50${\times2}$ as Teacher trained for 800 epochs. We note that the gain benefited from distillation becomes more distinct on smaller architectures and we further study the effect of various distilling sources in ablations.

% We also list results of distillation from a stronger \textit{SSL} pre-trained ResNet-50${\times2}$ model using {\large S}WAV with additional small patches utilized and trained for 800 epochs (see last row of Table~\ref{tbl:imgnet}), where EfficientNet-B0 further reaches 67.6\% Top-1 accuracy on ImageNet-1k. We introduce the details of using small patch views in Appendix. To test the distillation effect on larger student encoders, we also report the distillation results using ResNet-50 (see Appendix), and observe the same improvement trend: it reaches 74.3\%  Top-1 accuracy with  ResNet-50${\times2}$ as Teacher trained for 800 epochs. We note that the gain benefited from distillation becomes more distinct on smaller architectures and we further study the effect of various distilling sources in ablations.

\begin{figure}[t]
\centering
% \vspace{-2mm}
\includegraphics[width=.95\textwidth]{images/semi.pdf}
% \vspace{-4mm}
        \caption{\small ImageNet-1k Top-1 \textit{accuracy} for semi-supervised evaluations using 1\% (red line), 10\% (blue line) of the annotations for linear fine-tuning, in comparison with the fully supervised (green line) linear evaluation baseline for SEED. 
        For the points whose Teacher's number of parameters is at 0, we show the semi-supervised linear evaluation results of MoCo-V2 without any distillation. The Student models tend to perform better on the semi-supervised tasks after distillation from larger Teachers. }
        \label{fig:semi}
\vspace{-4mm}
\end{figure}
\noindent \textbf{Semi-Supervised Evaluation on ImageNet.} \;\; 
Following~\citep{oord2018representation,kornblith2019better,kolesnikov2019revisiting},
we evaluate the representation on the semi-supervised task, where a fixed 1\% or 10\% subsets of ImageNet training data~\citep{chen2020simple} are provided with the annotations.
After the self-supervised learning with and without distillation, we also train a classifier on top of the representation. 
The results are shown in Figure~\ref{fig:semi},
where the baseline without distillation is 
depicted when teacher parameters are 0.
As we can see, the accuracy is also improved
remarkably with {\large S}EED distillation, 
and a stronger teacher network with more parameters leads to a better performed student network. 
% We further evaluate the learned representations on the classification task using only a subset of ImageNet. We follow the semi-supervised learning protocol as in~\citep{oord2018representation,kornblith2019better,kolesnikov2019revisiting}, where the fixed 1\% and 10\% subsets of ImageNet labeled training data (provided by~\cite{chen2020simple}) are utilized for linear classification training. We report the Top-1 and Top-5 accuracy on the validation split in Figure~\ref{fig:semi}.

% We observe consistent with the results using the \textit{K}NN and semi-supervised evaluation protocols (see Figure~\ref{fig:semi}).




\noindent \textbf{Transferring to Classification.} To further study whether the improvement of the learned representations by distillation is confined to ImageNet, we evaluate on additional classification datasets to study the generalization and transferability of the feature representation. We follow the linear evaluation and fine-tuning settings as~\citep{kornblith2019better, chen2020simple, grill2020bootstrap}, that a linear layer is trained on the basis of frozen features. We report Top-1 Accuracy of models before and after distillation from various architectures on CIFAR-10, CIFAR-100~\citep{krizhevsky2009learning}, SUN-397~\citep{xiao2010sun} datasets (see Figure~\ref{fig:sun397}). More details regarding  pre-processing and training can be found in~\ref{sup:small}. Notably, we observe that our distillation surpasses contrastive self-supervised pre-training consistently on all benchmarks, verifying the effectiveness of {\large S}EED. This also proves the generalization ability of the learned representations from distillation to a wide range of data domain and different classes.

\noindent \textbf{Transferring to Detection and Segmentation.}
We conduct two downstream tasks here. The first is  
Faster R-CNN~\citep{ren2015faster} model for object detection trained on 
VOC-07+12 train+val set and evaluated on VOC-07 test split. 
The second is Mask R-CNN~\citep{he2017mask} model for the object detection and instance segmentation on COCO 2017 dataset~\citep{lin2014microsoft}.
The pre-trained model serves as the initial weight
and following~\cite{he2020momentum}, we fine-tune all the layers of the model.
More experiment settings can be found in~\ref{sup:detection}. 
The results are illustrated in Table~\ref{tbl:voc}.
As we can see, on VOC, the distilled pre-trained model achieves a large improvement. With ResNet-152 as the teacher network, the Resnet18-based Faster R-CNN model shows +0.7 point improvement on AP, +1.4 improvement on AP$_{50}$ and +1.6 on AP$_{75}$. 
On COCO, the improvement is relatively minor and the reason could be that COCO training set has $\sim$118k training images while VOC has only $\sim$16.5k training images. A larger training set with more fine-tuning iterations reduces the importance of the initial weights. 

%In order to comprehensively assess the transferability of the representations from {\large S}EED, we test it on different downstream tasks, \emph{e.g.}, object detection and segmentation. 
% Following~\cite{he2020momentum}, we fine-tune all the layers of a Faster R-CNN~\citep{ren2015faster} with C4-backbone on the VOC-07+12 train+val set, and evaluate it on VOC-07 test split. Specifically, the backbone in the detector contains only the convolutional layers from ResNet ending at conv4 stage, and the mask/box  prediction head consists of the conv5 stage (with a global pooling layer). Similarly, we use Mask R-CNN~\citep{he2017mask} with the C4 backbone for COCO segmentation. During training, we tune the Batch-Normalization layer as~\citep{he2020momentum}.  In Table~\ref{tbl:voc}, we list both the detection and segmentation results evaluated using  AP$_{50}$ and AP$_{75}$ (with threshold of IoU = 50\%, 75\%) and bounding box AP (AP$^{bb}$), mask AP (AP$^{mk}$). By distilling from larger architectures, {\large S}EED improves the results on the detection task: \textbf{+0.7} on AP, \textbf{+1.4} on AP$_{50}$ and \textbf{+1.6} on AP$_{75}$  than the MoCo-V2 baseline. Consistently, we observe same trend in segmentation results. Comparisons of performances using different backbones and the fine-tuning details can be found in the Appendix. 


% \input{tables/transfer}
% ~\ref{appendix:detection}
% \input{tables/coco_det_seg}

% Food-101~\cite{bossard2014food}, Caltech-101~\cite{griffin2007caltech} and Birdsnap~\cite{berg2014birdsnap} 

\input{tables/voc_det}

\begin{figure}[t]
\centering
% \vspace{-4mm}
\includegraphics[width=1.\textwidth]{images/CLS.pdf}
\vspace{-6mm}
\caption{\small ImageNet-1k \emph{Accuracy} (\%) of student network (EfficientNet-B0 and ResNet-18) transferred to other domains (CIFAR-10, CIFAR-100, SUN-397 datasets) with and without distillation from lager architectures (ResNet-50/101/152). }
\label{fig:sun397}
\vspace{-3mm}
\end{figure}

\input{tables/distill_imgnet_wider}

\subsection{Ablation Study}
We now explore the effects of distillation using different Teacher architectures, Teacher Pre-training algorithms, various distillation strategies and hyper-parameters.

\noindent \textbf{Different Teacher Networks.}  
Figure~\ref{fig:wider} summarizes the accuracy of ResNet-18 and EfficientNet-B0 distilled from wider and deeper ResNet architectures. We see clear performance improvement as depth and width of teacher network increase: compared to ResNet-50, deeper (ResNet-101) and wider (ResNet-50$\times$2) substantially improve the accuracy. However, further architectural enlargement has relatively limited effects, and we suspect
the accuracy might be limited by the student network capacity in this case.  

% In particular, Figure~\ref{fig:wider} summarizes the accuracy of ResNet-18 and EfficientNet-B0 distilling from wider ResNet architectures ($\times$1, $\times$2 parameters in ResBlock) when no small patches are used. We see clear performance improvement as depth and width of teacher network increase: comparing to ResNet-50, deeper (ResNet-101) and wider (ResNet-50$\times$2) substantially improve the accuracy. However, further architectural enlargement has relatively limited effects: ResNet-152$\times$2 does not obviously affect the performances.

\noindent \textbf{Different Teacher Pre-training Algorithms.} In Table~\ref{tbl:variants}, we show the Top-1 accuracy of ResNet-18 distilled from ResNet-50 with different pre-training algorithms, \textit{i.e.}, MoCo-V1~\citep{he2020momentum}, MoCo-V2~\citep{chen2020improved}, SimCLR~\citep{chen2020simple}, and {\large S}WAV~\citep{caron2020unsupervised}). 
Notably, the aforementioned methods all unanimously adopt contrastive-based pre-training except {\large S}WAV, which is based upon online clustering. We find that our {\large S}EED is agnostic to pre-training approaches, making it easy to use any self-supervised models (including clustering-based approach like {\large S}WAV) in self-supervised distillation. 
% Notably, We find that our {\large S}EED can improve the accuracy regardless of how the teacher is pre-trained, making it easy to use any self-supervised models in self-supervised distillation. 
In addition, we observe that more training epochs for both teacher \textit{SSL} and distillation epochs can bring beneficial gain. 



\noindent \textbf{Other Distillation Strategies.} 
We explore several alternative distillation strategies. \textit{l2-Distance}: where the \textit{l2}-distance of teacher \& student's embeddings are minimized, motivated by~\cite{romero2014fitnets}. 
\textit{$K$-Means}: we exploit \textit{K}-Means clustering to assign a pseudo-label based on the teacher network's representation.
\textit{Online Clustering}: we continuously update the clustering centers during distillation for pseudo-label generation. \textit{Binary Contrastive Loss}: we adopt an Info-NCE alike loss for contrastive distillation~\citep{tian2019contrastive}.
We provide details for other strategies in~\ref{sup:loss}.
Table~\ref{tbl:loss} shows the results for each method on  ResNet-18 (student) distilled from ResNet-50. From the results, the simple \textit{l2}-distance minimizing approach can achieve a decent accuracy, which demonstrates the effectiveness of applying the distillation idea to the self-supervised learning.  Beyond that, we study the effect of the original \textit{SSL} (MoCo-V2) supervision as supplementary loss to  {\large S}EED  and find it does not bring additional benefits to distillation. We find close results from these two strategies (Top-1 linear Acc.),  {\large S}EED  achieves 57.9\%, while SEED + MoCo-V2 achieves 57.6\%. 
This implies that the loss of  {\large S}EED can to a large extent cover the original \textit{SSL} loss, and it is not necessary to conduct \textit{SSL} any further during distillation. 
Meanwhile, our proposed SEED outperforms these alternatives with highest accuracy, which shows the superiority of aligning the student towards the teacher and contrasting with the irrelevant samples. 

% We compare {\large S}EED with several other distillation strategies, which include minimizing the \textit{l2}-distance of embeddings, pseudo-label classification using \textit{K}-Means Clustering, online clustering, and the contrastive-akin distillation method CRD~\citep{tian2019contrastive} in Table~\ref{tbl:loss}. It's worth noting that simply minimizing the \textit{l2}-distance between student as teacher's visual embeddings yields a decent performance: 55.3\% on ImageNet validation split using ResNet-18 as the student and a pre-trained ResNet-50 as the teacher. This observation aligns with the conclusion in~\citep{grill2020bootstrap}, where the visual representation is trained by learning to mimic the representations of just augmented views of positive samples. \textit{K}-Means Clustering constructs pseudo-labels as cross-entropy targets by clustering features from the teacher encoder in an offline manner. In practice, we find that when a smaller number of \textit{K} is set, the assigned categorical center for a sample can be samples assigned with the same label are quite different from each other and should be further discriminated. Thus, in contrary to \textit{l2}-distance, \textit{K}-Means clustering innately lays particular emphasis on discriminating different samples rather than aligning different views from identical images. In particular, we note that CDR is a variation of contrastive distillation by minimizing an upper-bound of \textit{Info-NCE} objectiveness~\citep{oord2018representation}, but it was designed to facilitate supervised distillation. We apply it on our self-supervised distillation task as a binary form of \textit{Info-NCE} loss, therefore it is expected to produce a close result with {\large S}EED.

\noindent \textbf{Other Hyper-Parameters.}  
Table~\ref{tbl:negtive} summarizes the distillation performances on multiple datasets using different temperature $\tau^{T}$.
%If $\tau^T$ is small, the similarity distribution of $p^T$ tends to be a one-hot vector, and the distillation process requires the student feature to be dissimilar with the samples in the queue. On contrary, if $\tar^T$ is large, the normalized similarity score of $p_j^T$ with the samples in the queue tends to be large and requires the student feature to be more similar.
%As the results shown, the accuracy increases first and then drops when we decrease the value.
We observe a better performance when decreasing $\tau^{T}$ to 0.01 for ImageNet-1k and CIFAR-10 dataset, and to 1e-3 for CIFAR-100 datasets. When $\tau$ is large, the softmax-normalized similarity score of $p_j^T$ between $\mathbf{z}_i^T$ and instance $\mathbf{d}_j$ in the queue $\mathbf{D}^+$ also becomes large, which means the student's feature should be less discriminative with the features of other images to some extent. When $\tau^{T}$ is 0, the teacher model will generate a one-hot vector, which only treats $\mathbf{z}_i^T$ as a positive instance and all others in the queue as negative.
Thus, the best $\tau$ is a trade-off depending on the data distribution.
We further compare effect of different hyper-parameters in~\ref{sup:ablation}.




\input{tables/distill_loss}


==> ICLR20_Distillatio (2)/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> ICLR20_Distillatio (2)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
% \DeclareMathOperator*{\log}{\text{log}}
% \DeclareMathOperator*{\exp}{\text{exp}}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}%
\definecolor{cellcolor}{RGB}{163, 240, 247}


%Sup code

\usepackage[utf8]{inputenc}

\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.3,0.6,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{maroon}{RGB}{251,57,157}
\definecolor{p}{RGB}{148,2,209}
\definecolor{keyword}{RGB}{184,86,225}
\definecolor{backcolour}{rgb}{255, 255, 255}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegray},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    % moredelim=**[is][\color{red}]{~}{~},
    moredelim = [s][\color{purple}]{\\[}{\\]},
}



==> ICLR20_Distillatio (2)/method.tex <==
\section{Method}


==> ICLR20_Distillatio (2)/packages.tex <==
\usepackage{epsfig}
\usepackage{graphicx}

\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}

\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}
\usepackage{enumerate}

\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}

\usepackage{booktabs}
\usepackage{longtable}
\usepackage{arydshln}
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
%\usepackage[table]{xcolor}% http://ctan.org/pkg/xcolor
\usepackage{xcolor}% http://ctan.org/pkg/xcolor
\usepackage{hyperref}
\hypersetup{colorlinks,linkcolor={red},citecolor={blue},urlcolor={red}}  
% \usepackage[export]{adjustbox}

% Table float box with bottom caption, box width adjusted to content
\usepackage[T1]{fontenc}
\usepackage[font=small,labelfont=bf,tableposition=top]{caption}

\DeclareCaptionLabelFormat{andtable}{#1~#2  \&  \tablename~\thetable}
\usepackage{capt-of}% or \usepackage{caption}
\usepackage{hyperref}
 \usepackage{relsize}
\usepackage{bbold}
\usepackage{epigraph}
\usepackage{diagbox}
\usepackage{makecell}
\usepackage{xr}
\usepackage{xr-hyper}


==> ICLR20_Distillatio (2)/relatedwork.tex <==
\section{Related Work} 
Among the recent literature in self-supervised learning, contrastive based approaches show prominent results on downstream tasks. Majority of the techniques along this direction are stemming from noise-contrastive estimation~\citep{gutmann2010noise} where the latent distribution is estimated by contrasting with randomly or artificially generated noises. 
% Variations of this idea have been successfully applied to series of tasks, \textit{e.g.}, language embedding~\citep{mnih2013learning}, audio classification~\citep{oord2018representation}, face recognition~\citep{sun2014deep}, and so forth.
~\cite{oord2018representation} first proposed Info-NCE to learn image representations by predicting the future using an auto-regressive model for unsupervised learning. Follow-up works include improving the efficiency~\citep{henaff2019data}, and using multi-view as positive samples~\citep{tian2019contrastive1}. As these approaches can only have the access to limited negative instances,~\cite{wu2018unsupervised} designed a memory-bank to store the previously seen random representations as negative samples, and treat each of them as independent categories (instance discrimination). However, this approach also comes with a deficiency that the previously stored vectors are inconsistent with the recently computed representations during the earlier stage of pre-training. ~\cite{chen2020simple} mitigate this issue by sampling negative samples from a large batch. Concurrently,~\cite{he2020momentum} improve the memory-bank based method and propose to use the momentum updated encoder for the remission of representation inconsistency. Other techniques include~\cite{misra2020self} that combines the pretext-invariant objective loss with contrastive learning, and ~\cite{wang2020understanding} that decomposes contrastive loss into alignment and uniformity objectiveness.


Knowledge distillation~\citep{hinton2015distilling} aims to transfer knowledge from a cumbersome model to a smaller one without losing too much generalization power, which is also well investigated in model compression~\citep{bucilua2006model}. Instead of mimicking the teacher's output logit, attention transfer~\citep{zagoruyko2016paying} formulates knowledge distillation on attention maps. Similarly, works in ~\citep{ahn2019variational,yim2017gift,koratana2019lit,huang2017like} have utilized different learning objectives including consistency on feature maps, consistency on probability mass function, and maximizing the mutual information. CRD~\citep{tian2019contrastive}, which is derived from CMC~\citep{tian2019contrastive1}, optimizes the student network by a similar objective to~\cite{oord2018representation} using a derived lower bound on mutual information. 
However, the aforementioned efforts all focus on task-specific distillation (\textit{e.g.}, image classification) during the fine-tuning phase  rather than a task-agnostic distillation in the pre-training phase for the representation learning. Several works on natural language pre-training proposed to leverage knowledge distillation for a smaller yet stronger small models. For instances, DistillBert~\citep{sanh2019distilbert}, TinyBert~\citep{jiao2019tinybert}, and MobileBert~\citep{sun2020mobilebert}, have used knowledge distillation for model compression and shown their validity on multiple downstream tasks. Similar works also emphasize the value of smaller and faster models for language representation learning by leveraging knowledge distillation~\citep{turc2019well, sun2019patient}. These works all demonstrate the effectiveness of knowledge distillation for language representation learning in small models, while are not extended to the pre-training for visual representations. Notably, a recent concurrent work CompRess~\citep{abbasi2020compress} also point out the importance to develop better \textit{SSL} method for smaller models.
%importance to distill for small models; 
{\large S}EED closely relates to the above techniques but aims to facilitate \textbf{visual representation learning during pre-training phase using distillation technique for small models}, which as far as we know has not yet been investigated.

% consider to remove task-agnostic distillation this term.
% Fine-tuning phrase distillation, not conflict with our setting
% but it may request more cost (e.g., label collection)

% (1) Turc, I.; Chang, M.-W.; Lee, K.; Toutanova, K. Well-Read Students Learn Better: On the Importance of Pre-Training Compact Models. arXiv:1908.08962 [cs] 2019.

% (3) Tsai, H.; Riesa, J.; Johnson, M.; Arivazhagan, N.; Li, X.; Archer, A. Small and Practical BERT Models for Sequence Labeling. arXiv:1909.00100 [cs] 2019.

% (4) Sun, S.; Cheng, Y.; Gan, Z.; Liu, J. Patient Knowledge Distillation for BERT Model Compression. arXiv:1908.09355 [cs] 2019.


% (6) Wang, W.; Wei, F.; Dong, L.; Bao, H.; Yang, N.; Zhou, M. MiniLM: Deep Self-Attention Distillation for Task-Agnostic Compression of Pre-Trained Transformers. arXiv:2002.10957 [cs] 2020.


==> ICLR20_Distillatio (2)/tables/coco_det_seg.tex <==
% \begin{table}[t]

% %   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

% \setlength{\tabcolsep}{3pt}
% \begin{center}
% \renewcommand{\arraystretch}{1.2} % Default value: 1
% \begin{tabular}{ccccccccccc}
% \toprule
% \\[-3.5ex]
% \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multicolumn{3}{c}{\textbf{VOC07 Detection}} & \multicolumn{3}{c}{\textbf{COCO Detection}} & \multicolumn{3}{c}{\textbf{COCO Inst. Segment.}} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8} \cmidrule(lr){9-11}\\[-3.5ex]
%  &  & AP^{\text{bb}}  & AP^\text{bb}_{50}  & AP^\text{bb}_{75} & AP^{\text{bb}}  & AP^\text{bb}_{50}  & AP^\text{bb}_{75} & AP^{\text{mk}}  & AP^\text{mk}_{50}  & AP^\text{mk}_{75}\\
%  \\[-3.5ex]
% \midrule
% R18 & \xmark 	& 46.1 & 74.5 & 48.6 & 32.2 & 50.7 & 34.2 & 28.9 & 48.0 & 30.5 \\
% R34 & \xmark 	& 53.6 & 79.1 & 58.7 &  & &  \\
% R50 & \xmark 	& 57.0 & 82.4 & 63.6 & 35.6 & 57.3 & 37.6 & 40.7 & 60.5 & 44.1\\
% % ResNet101 & \xmark 	& \\
% % ResNet152 & \xmark 	 \\
%  \hdashline \\[-3ex]
 
% \multirow{3}{*}{{R18}} & R50 	& 46.1 {\scriptsize ( 0.0)} & 74.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 49.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & R101 	& 46.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 75.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+1.3})}$} & 49.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 32.4{\scriptsize (+0.2)} & 51.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 34.5{\scriptsize (+0.3)} & 29.1{\scriptsize (+0.2)}&  48.2{\scriptsize (+0.2)} &  30.5{\scriptsize ( 0.0)}\\
%  & R152 	& \\
% \hdashline \\[-3ex]

% \multirow{3}{*}{{R34}} & R50 	& 53.7  {\scriptsize (+0.1)}& 79.4 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$}  & 59.2 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & R101 	&  54.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$} & 79.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 59.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$}\\
%  & R152 	& \\
% \hdashline \\[-3ex]

% \multirow{3}{*}{{R50}} & R50 	& \\
%  & R101 	&  57.1 {\scriptsize (+0.1)} & 82.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 63.8  {\scriptsize (+0.2)}\\
%  & R152 	& \\


% \toprule
% \end{tabular}
% \caption{
% {\small
% Object detection and instance segmentation fine-tuned on VOC07 and COCO: bounding-box AP (AP$^{bb}$) and mask AP (AP$^{mk}$) evaluated
% on VOC07-val and COCO-val2017 respectively. The first several rows show the baselines from unsupervised backbones without distillation. R* represents the ResNet\{18, 32, 50\} architectures.
% }}
% \label{tbl:cifar100_diff}
% \end{center}
% \vspace{-10pt}
% \end{table}

\begin{table}[t]
\setlength{\tabcolsep}{6pt}
\begin{center}
\renewcommand{\arraystretch}{1.2} % Default value: 1
{\small
\begin{tabular}{ccccccccccc}
\toprule
\\[-3.5ex]
\multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} & \multicolumn{3}{c}{\textbf{Object Detection}} & \multicolumn{3}{c}{\textbf{Instance Segmentation}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8} \cmidrule(lr){9-11}\\[-3.5ex]
 &  & AP$^{\text{bb}}$  & AP$^\text{bb}_{50}$  & AP$^\text{bb}_{75}$ & AP$^{\text{mk}}$  & AP$^\text{mk}_{50}$  & AP$^\text{mk}_{75}$\\
 \\[-3.5ex]
\midrule
ResNet18 & \xmark  & 32.2 & 50.7 & 34.2 & 28.9 & 48.0 & 30.5 \\
ResNet34 & \xmark  &  & &  \\
ResNet50 & \xmark  & 35.6 & 57.3 & 37.6 & 40.7 & 60.5 & 44.1\\
% ResNet101 & \xmark 	& \\
% ResNet152 & \xmark 	 \\
 \hdashline \\[-3ex]
 
\multirow{3}{*}{{ResNet18}} & ResNet50 \\
 & ResNet101 	& 32.4{\scriptsize (+0.2)} & 51.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 34.5{\scriptsize (+0.3)} & 29.1{\scriptsize (+0.2)}&  48.2{\scriptsize (+0.2)} &  30.5{\scriptsize ( 0.0)}\\
 & ResNet152 	& \\
\hdashline \\[-3ex]

\multirow{3}{*}{{ResNet34}} & ResNet50 \\
 & ResNet101 	& \\
 & ResNet152 	& \\
\hdashline \\[-3ex]

\multirow{3}{*}{{ResNet50}} & ResNet50 	& \\
 & ResNet101 	& \\
 & ResNet152 	& \\
\toprule
\end{tabular}
}
\caption{
{\small
Object detection and instance segmentation fine-tuned on COCO: bounding-box AP (AP$^{bb}$) and mask AP (AP$^{mk}$) evaluated
on VOC07-val and COCO-val2017 respectively. The first several rows show the baselines from unsupervised backbones without distillation. 
}}
\label{tbl:cifar100_diff}
\end{center}
\vspace{-10pt}
\end{table}


==> ICLR20_Distillatio (2)/tables/distill_imgnet.tex <==
% \begin{table}[ht]

% %   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

% \setlength{\tabcolsep}{4.pt}
% \begin{center}
% \renewcommand{\arraystretch}{1.2} % Default value: 1
% \begin{tabular}{llcccccccc}
% \toprule
% \\[-3.5ex]
% \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multicolumn{2}{c}{\textbf{Student}} & \multicolumn{2}{c}{\textbf{Teacher}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{2}{c}{\textbf{Linear}} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-9}\\[-3.5ex]
%  & & \textbf{KNN}  & \textbf{Linear}  & \textbf{KNN}  & \textbf{Linear} & Top-1 & Top-1 & Top-5\\
%  \\[-3.5ex]
% \midrule
% \multirow{3}{*}{MobileNet-v3} & ResNet50& \multirow{3}{*}{21.4} &  \multirow{3}{*}{-} & 46.0 & 67.4  & 41.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+19.7})}$}	& -	& -\\
%  & ResNet101 & & & 52.0 & 70.3 & -	& - & -\\
%  & ResNet152 &  & & -  & -	& - & - & -\\
%  \hdashline \\[-3ex]
 
 
% \multirow{3}{*}{ResNet18} & ResNet50& \multirow{3}{*}{36.7}  & \multirow{3}{*}{52.5} & 46.0& 67.4  & 43.4 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+6.7})}$}	& - & -\\
%  & ResNet101	&  &  &52.0 & 70.3  & 48.6 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+11.9})}$}	& 58.9 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+6.4})}$} & -\\
%  & ResNet152	&  &  & -  &-  & -& - & -\\ \\[-3ex]
% \hdashline \\[-3ex]


% \multirow{3}{*}{ResNet34} & ResNet50&  \multirow{3}{*}{41.5} &  \multirow{3}{*}{57.4} & 46.0 & 67.4  & 45.2 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+3.7})}$}	& - & -\\
%   & ResNet101	&  &  & 52.0 & 70.3  & 50.5 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+9.0})}$}	& 61.6 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+4.2})}$}	& -\\
%   & ResNet152	&  &  & - & -  &-	& -	& -\\
% \hdashline \\[-3ex]


% \multirow{3}{*}{ResNet50} & ResNet50&  \multirow{3}{*}{46.0} &  \multirow{3}{*}{67.4} & 46.6 & - & - & -\\
%   & ResNet101	&  &  & 52.0 & 70.3  & - 	& 69.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+1.7})}$}	& -\\
%   & ResNet152	&  &  & - & -  &-	& -	& -\\
% % $\mathcolor{red}{\downarrow}$
% \toprule
% \end{tabular}
% \caption{
% {
% Top-1 test \emph{accuracy} (\%) of student networks on ImageNet-1k for transfer across multiple \emph{deeper} teacher and student architectures.
% }}
% \label{tbl:cifar100_diff}
% \end{center}
% \vspace{-10pt}
% \end{table}




% \begin{table}[h]
% % \vspace{-3mm}
% %   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

% \setlength{\tabcolsep}{5.pt}
% \begin{center}
% \renewcommand{\arraystretch}{1.} % Default value: 1
% {
% \small
% \scalebox{0.95}{
% \begin{tabular}{ccccccccc}
% \toprule
% \\[-2.8ex]
% \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} & \multicolumn{1}{c}{\textbf{\textit{K}NN}} & \multicolumn{2}{c}{\textbf{Linear-100\%}} & \multicolumn{2}{c}{\textbf{Semi-1\%}} & \multicolumn{2}{c}{\textbf{Semi-10\%}}\\
% \cmidrule(lr){3-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}\\[-2.8ex]
%  & & Top-1 & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5\\
%  \\[-3.1ex]
% \midrule
% % ResNet34& \xmark & 41.5 & - & 57.4 & -\\
% % ResNet50& \xmark & 46.0 & - & 67.4 & - \\ 
% % ResNet101& \xmark & 52.0 & - & 70.3 & -\\ 
% % ResNet152& \xmark & - & -\\ 

%  \multirow{4}{*}{
% EfficientNet-b0}&  \xmark &  & 39.1 & 64.6 &  & & \\
%  & ResNet-50  & 46.0 &  61.3 & 82.7 & 37.7 & 62.4 & 53.2 & 76.0 \\
%  & ResNet-101 &	50.1 & 63.0 & 83.8 & 41.3 & 65.5 & 55.8 & 78.0\\
%  & ResNet-152 & 50.7 & 65.3 & 86.0 & 41.7 & 67.0 & 56.5  & 79.0\\[.2ex]
%  \hdashline \\[-1.9ex]
 
 
% %  \hdashline \\[-2.5ex]
% \multirow{4}{*}{
% MobileNet-v3}&  \xmark & 27.5 & 36.3 & 62.2 & 18.3 & 38.4 & 32.4& 55.4 \\
%  & ResNet-50  & 44.8 & 55.2 & 80.3 & 36.2 & 62.0  & 51.7 & 75.8  \\
%  & ResNet-101 & 48.8 & 59.9 & 83.5 & 38.3 & 64.0 & 52.8 & 76.2  \\
%  & ResNet-152 & 49.5 & 61.4 & 84.6 & 38.9 & 63.9 & 52.8 & 75.9 \\[.2ex]
%  \hdashline \\[-1.9ex]
 
 
% \multirow{4}{*}{
% ResNet-18} & \xmark & 36.7 & 52.5 & 77.0 & 30.9 & 57.9 & 45.6 & 72.4 \\
%  & ResNet-50 & 43.4 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+ 6.7})}$} & 57.6 & 81.8 & \\
%  & ResNet-101  & 48.6 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+11.9})}$} & 58.9 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+ 6.4})}$} & 82.5 & 41.8 &68.1 & 52.2 & 77.6 \\
%  & ResNet-152& 49.1 & 59.5 & 83.3 & 44.1 & 71.0 & 54.6 & 79.6 \\[.2ex]
% \hdashline \\[-1.9ex]


% \multirow{4}{*}{
% ResNet-34}& \xmark & 41.5 & 57.4 & 81.6\\
%   & ResNet-50&  45.2 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+ 3.7})}$} & 58.5 & 82.6\\
%   & ResNet-101 & 50.5  & 61.6 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+ 4.2})}$}	&  84.9\\
%   & ResNet-152 & 51.4	& 62.7 & 85.8 \\[.2ex]
% \hdashline \\[-1.9ex]


% \multirow{5}{*}{
% ResNet-50}& \xmark & 46.1  & 67.4 & 87.8 \\ 
%   & ResNet-50 &  46.1 & 67.5 & 87.8\\
%   & ResNet-101 & 52.3 	& 69.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+ 1.7})}$} & 88.7\\
%   & ResNet-152	 & 53.2 	&  70.4 & 90.5 \\
%   & ResNet-50$\times$2^{*}	 & 54.0	&  74.3 & 92.2 \\
% % $\mathcolor{red}{\downarrow}$
% \toprule
% \end{tabular}
% }
% }
% \caption{
% {\small
% ImageNet-1k top-1/5 test \emph{accuracy} (\%) under linear classification, \textit{K}NN and semi-supervised linear evaluation across multiple students and \emph{deeper} teacher architectures. \xmark\, denotes MoCo-V2 self-supervised learning baselines before distillation. * indicates the teacher encoder is pre-trained using SWAV and distillation contains additional small-patches.
% % \jianfw{how about split the table into two tables. one is for knn and linear probe. the other is for semi-supervised. Meanwhile, also discuss the two settings seperatly.}
% }}
% \label{tbl:imgnet}
% \end{center}
% \vspace{-8mm}
% \end{table}


% \begin{table}[t]
% % \vspace{-3mm}
% %   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

% \setlength{\tabcolsep}{4.6pt}
% \begin{center}
% \renewcommand{\arraystretch}{1.07} % Default value: 1
% {
% \small
% \scalebox{0.94}{
% \begin{tabular}{cccccccccccccccc} 
% % \hline
% \toprule
% % \Xhline{3\arrayrulewidth}   \cmidrule(lr){14-1
% \\[-2.8ex]
% \multirow{2}{*}{\backslashbox{\textbf{T}}{\textbf{S}}} &   \multicolumn{3}{@{\vline}c@{\vline}}{\textbf{Eff-b0}} &
% \multicolumn{3}{c@{\vline}}{\textbf{Eff-b1}} & \multicolumn{3}{c@{\vline}}{\textbf{Mob-v3}} & \multicolumn{3}{c@{\vline}}{\textbf{R-18}} & \multicolumn{3}{c}{\textbf{R-34}}   \\
% %  \cline{2-4}  \cline{5-7}  \cline{8-10}  \cline{11-13}   \cline{14-16}  
%  & \multicolumn{1}{@{\vline}c}{\textit{K}} & T-1 &  \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & T-5 \\
%  \hline
%  \\[-2.0ex]
% % \hline \\[-2.ex]
%  \xmark & 30.0 & 42.2 & \multicolumn{1}{c}{68.5}  & 34.4  & 50.7 & 74.6 & 27.5 & 36.3 & 62.2 & 36.7 & 52.5 & 77.0 & 41.5 & 57.4 & 81.6 \\[.2ex] 
%  \hdashline \\[-1.9ex]
%  \multirow{1}{*}{\textbf{R-50}} & 46.0 & 61.3 & 82.7 & 46.1 & 61.4 & 83.1   & 44.8 & 55.2 & 80.3 & 43.4 & 57.6 & 81.8 & 45.2 & 58.5 & 82.6 \\[-.8ex]
%  {\tiny $\Delta$}& {\tiny $\mathcolor{darkgreen}{\textbf{+16.0}}$}  & {\tiny $\mathcolor{darkgreen}{\textbf{+19.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+14.2}}$}  & {\tiny $\mathcolor{darkgreen}{\textbf{+16.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+10.7}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+8.8}}$}&	{\tiny $\mathcolor{darkgreen}{\textbf{+17.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.9}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+5.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+4.8}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+3.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+1.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+1.0}}$} 
% \\[.2ex] 
% \hdashline \\[-1.9ex]
%   \multirow{1}{*}{\textbf{R-101}} & 50.1 & 63.0 & 83.8  & 50.3 &  &  & 48.8 & 59.9 & 83.5 & 48.6 & 58.9 & 82.5 & 50.5 & 61.6 & 84.9 \\[-.8ex]
%  {\tiny $\Delta$} & {\tiny $\mathcolor{darkgreen}{\textbf{+20.1}}$}  & {\tiny $\mathcolor{darkgreen}{\textbf{+20.8}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+15.3}}$}  & 
%  {\tiny $\mathcolor{darkgreen}{\textbf{+15.9}}$} &
%  {\tiny $\mathcolor{darkgreen}{\textbf{}}$}
%  &
%  {\tiny $\mathcolor{darkgreen}{\textbf{}}$}
%  &	{\tiny $\mathcolor{darkgreen}{\textbf{+21 .3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+23.6}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+21.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+11.9}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.4}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+5.5}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+9.0}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+4.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+3.3}}$}
%  \\[.2ex]
%  \hdashline \\[-1.9ex]
%   \multirow{1}{*}{\textbf{R-152}}& 50.7 & 65.3 & 86.0  & 52.4 & 67.3 & 86.9  & 49.5 & 61.4 & 84.6 & 49.1 & 59.5 & 83.3 & 51.4 & 62.7 & 85.8 \\[-.8ex]
%  {\tiny $\Delta$} & {\tiny $\mathcolor{darkgreen}{\textbf{+20.7}}$}  & {\tiny$\mathcolor{darkgreen}{\textbf{+23.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+17.5}}$} & 
%  {\tiny $\mathcolor{darkgreen}{\textbf{+18.0}}$}&
%  {\tiny $\mathcolor{darkgreen}{\textbf{+16.6}}$}&
%  {\tiny $\mathcolor{darkgreen}{\textbf{+12.3}}$}&	{\tiny$\mathcolor{darkgreen}{\textbf{+22.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+25.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+22.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+12.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+7.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+6.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+9.9}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+5.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+4.2}}$} 
%  \\[.2ex] 
%  \hdashline \\[-1.9ex]
%   \multirow{1}{*}{\textbf{R50{\tiny $\times$2}^{*}}} & 57.4 & 67.6 & 87.4  & 60.3  & 67.8 & 87.6 & 55.9 & 68.2 & 88.2 & 55.3 & 63.0 & 84.9 &  58.2 & 65.7 & 86.8  \\[-.8ex]
%  {\tiny $\Delta$} & {\tiny$\mathcolor{darkgreen}{\textbf{+27.4}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+25.4}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+28.4}}$}  &
%  {\tiny $\mathcolor{darkgreen}{\textbf{+25.9}}$}&
%  {\tiny $\mathcolor{darkgreen}{\textbf{+17.1}}$} & 
%  {\tiny $\mathcolor{darkgreen}{\textbf{+13.0}}$}& {\tiny$\mathcolor{darkgreen}{\textbf{+18.9}}$} & 
%  {\tiny$\mathcolor{darkgreen}{\textbf{+31.9}}$} & 
%  {\tiny$\mathcolor{darkgreen}{\textbf{+26.0}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+18.6}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+10.5}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+7.9}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+16.7}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+8.3}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+5.2}}$} &
% % \Xhline{3\arrayrulewidth}
% % STess eff-b0 size of input is 224 (not 256)
% \bottomrule
% \end{tabular}}}
% \vspace{1mm}
% \caption{
% {\small
% ImageNet-1k test \emph{accuracy} (\%) using \textit{K}NN and linear classification for multiple students and MoCo-v2 pre-trained \emph{deeper} teacher architectures. \xmark\, denotes MoCo-V2 self-supervised learning baselines before distillation. * indicates using a deeper teacher encoder pre-trained by {\normalsize S}WAV, where additional small-patches are also utilized during distillation and trained for 800 epochs. \textit{K} denotes Top-1 accuracy using \textit{K}NN. T-1 and T-5 denote Top-1 and Top-5 accuracy using linear evaluation.
% }}
% \label{tbl:imgnet}
% \end{center}
% \vspace{-8mm}
% \end{table}
% image size 256, ablation, and stress this setting


\begin{table}[t]
% \vspace{-3mm}
%   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

\setlength{\tabcolsep}{4.1pt}
\begin{center}
\renewcommand{\arraystretch}{1.07} % Default value: 1
\caption{
{\small
ImageNet-1k test \emph{accuracy} (\%) using \textit{K}NN and linear classification for multiple students and MoCo-v2 pre-trained \emph{deeper} teacher architectures. \xmark\, denotes MoCo-V2 self-supervised learning baselines before distillation. * indicates using a deeper teacher encoder pre-trained by {\normalsize S}WAV, where additional small-patches are also utilized during distillation and trained for 800 epochs. \textit{K} denotes Top-1 accuracy using \textit{K}NN. T-1 and T-5 denote Top-1 and Top-5 accuracy using linear evaluation. First column shows Top-1 Acc. of Teacher network. First row shows the supervised performances of student networks.
}}
% \vspace{-2mm}
{
\small
\scalebox{0.92}{
\begin{tabular}{ccccccccccccccccc} 
% \hline
\toprule
\\[-2.8ex]
\multirow{2}{*}{\backslashbox{\textbf{T}}{\textbf{S}}} & 
\multirow{2}{*}{T-1}
&\multicolumn{3}{@{\vline}c@{\vline}}{\textbf{Eff-b0}} &
\multicolumn{3}{c@{\vline}}{\textbf{Eff-b1}} & \multicolumn{3}{c@{\vline}}{\textbf{Mob-v3}} & \multicolumn{3}{c@{\vline}}{\textbf{R-18}} & \multicolumn{3}{c}{\textbf{R-34}}   \\
 & & \multicolumn{1}{@{\vline}c}{\textit{K}} & T-1 &  \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & \multicolumn{1}{c@{\vline}}{T-5} & \textit{K} & T-1 & T-5 \\
 \hline
 \\[-2.0ex]
% \hline \\[-2.ex]
 \multicolumn{2}{c}{\textbf{Supervised Acc.}} &  & 77.3 &  &  & 79.2  &   &  & 75.2  &   &  & 69.5  &  & & 72.8 & \\[.2ex] 
 \hdashline \\[-1.9ex]
 \xmark & - & 30.0 & 42.2 & \multicolumn{1}{c}{68.5}  & 34.4  & 50.7 & 74.6 & 27.5 & 36.3 & 62.2 & 36.7 & 52.5 & 77.0 & 41.5 & 57.4 & 81.6 \\[.2ex] 
 \hdashline \\[-1.9ex]
 \multirow{1}{*}{\textbf{R-50}} &  \multirow{2}{*}{67.4} & 46.0 & 61.3 & 82.7 & 46.1 & 61.4 & 83.1   & 44.8 & 55.2 & 80.3 & 43.4 & 57.9 & 82.0 & 45.2 & 58.5 & 82.6 \\[-.8ex]
 {\tiny $\Delta$}&  &{\tiny $\mathcolor{darkgreen}{\textbf{+16.0}}$}  & {\tiny $\mathcolor{darkgreen}{\textbf{+19.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+14.2}}$}  & {\tiny $\mathcolor{darkgreen}{\textbf{+16.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+10.7}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+8.8}}$}&	{\tiny $\mathcolor{darkgreen}{\textbf{+17.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.9}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+5.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+4.8}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+3.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+1.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+1.0}}$} 
\\[.2ex] 
\hdashline \\[-1.9ex]
  \multirow{1}{*}{\textbf{R-101}} & \multirow{2}{*}{70.3} & 50.1 & 63.0 & 83.8  & 50.3 & 63.4 & 84.6 & 48.8 & 59.9 & 83.5 & 48.6 & 58.9 & 82.5 & 50.5 & 61.6 & 84.9 \\[-.8ex]
 {\tiny $\Delta$} & & {\tiny $\mathcolor{darkgreen}{\textbf{+20.1}}$}  & {\tiny $\mathcolor{darkgreen}{\textbf{+20.8}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+15.3}}$}  & 
 {\tiny $\mathcolor{darkgreen}{\textbf{+15.9}}$} &
 {\tiny $\mathcolor{darkgreen}{\textbf{+12.7}}$}
 &
 {\tiny $\mathcolor{darkgreen}{\textbf{+10.0}}$}
 &	{\tiny $\mathcolor{darkgreen}{\textbf{+21 .3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+23.6}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+21.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+11.9}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.4}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+5.5}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+9.0}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+4.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+3.3}}$}
 \\[.2ex]
 \hdashline \\[-1.9ex]
  \multirow{1}{*}{\textbf{R-152}}& \multirow{2}{*}{74.2} & 50.7 & 65.3 & 86.0  & 52.4 & 67.3 & 86.9  & 49.5 & 61.4 & 84.6 & 49.1 & 59.5 & 83.3 & 51.4 & 62.7 & 85.8 \\[-.8ex]
 {\tiny $\Delta$} & &{\tiny $\mathcolor{darkgreen}{\textbf{+20.7}}$}  & {\tiny$\mathcolor{darkgreen}{\textbf{+23.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+17.5}}$} & 
 {\tiny $\mathcolor{darkgreen}{\textbf{+18.0}}$}&
 {\tiny $\mathcolor{darkgreen}{\textbf{+16.6}}$}&
 {\tiny $\mathcolor{darkgreen}{\textbf{+12.3}}$}&	{\tiny$\mathcolor{darkgreen}{\textbf{+22.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+25.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+22.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+12.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+7.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+6.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+9.9}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+5.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+4.2}}$} 
 \\[.2ex] 
 \hdashline \\[-1.9ex]
  \multirow{1}{*}{\textbf{R50{\tiny $\times$2}$^{*}$}} & \multirow{2}{*}{77.3} & 57.4 & 67.6 & 87.4  & 60.3  & 68.0 & 87.6 & 55.9 & 68.2 & 88.2 & 55.3 & 63.0 & 84.9 &  58.2 & 65.7 & 86.8  \\[-.8ex]
 {\tiny $\Delta$} & &{\tiny$\mathcolor{darkgreen}{\textbf{+27.4}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+25.4}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+18.9}}$}  &
 {\tiny $\mathcolor{darkgreen}{\textbf{+25.9}}$}&
 {\tiny $\mathcolor{darkgreen}{\textbf{+17.3}}$} & 
 {\tiny $\mathcolor{darkgreen}{\textbf{+13.0}}$}& {\tiny$\mathcolor{darkgreen}{\textbf{+18.9}}$} & 
 {\tiny$\mathcolor{darkgreen}{\textbf{+31.9}}$} & 
 {\tiny$\mathcolor{darkgreen}{\textbf{+26.0}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+18.6}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+10.5}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+7.9}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+16.7}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+8.3}}$} & {\tiny$\mathcolor{darkgreen}{\textbf{+5.2}}$} \\
\bottomrule
\end{tabular}}}
\vspace{1mm}
\label{tbl:imgnet}
\end{center}
% \vspace{-2mm}
\end{table}

==> ICLR20_Distillatio (2)/tables/distill_imgnet_wider.tex <==

% \begin{table}[!htb]
% \begin{minipage}{.48\linewidth}
%     \centering
%     \medskip
%         \setlength{\tabcolsep}{3.4pt}
%         \small
%         \begin{tabular}{cccccc}
%             \toprule
%             \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multirow{2}{*}{\textbf{Width}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{2}{c}{\textbf{Linear}} \\
%             \cmidrule(lr){4-4}\cmidrule(lr){5-6}
%              &  & & Top-1 & Top-1 & Top-5\\
%             \midrule
            
%             \multirow{5}{*}{R18} & \xmark & - & 46.0 & 67.4 & -  \\
%               & R50 	& 1 & 46.6 & - & - \\
%               & R50 	& 2 & \\
%               & R101 	& 1 & - & 69.1\\
%               & R101    & 2 \\
%             \toprule
%         \end{tabular}
%         \caption{\small \emph{Accuracy} of student network (ResNet50) on ImageNet-1k distilled from teacher networks with different widths.}
%         \label{tab:first_table}
%     \end{minipage}\hfill
%     \begin{minipage}{.48\linewidth}
%         \centering
%         \medskip
%         \setlength{\tabcolsep}{3.4pt}
%         \small
%         \begin{tabular}{cccccc}
%             \toprule
%             \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multirow{2}{*}{\textbf{Epochs}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{2}{c}{\textbf{Linear}} \\
%             \cmidrule(lr){4-4}\cmidrule(lr){5-6}
%              &  & & Top-1 & Top-1 & Top-5\\
%             \midrule
            
%             \multirow{4}{*}{R18} & R50& 200 & 46.6 \\
%               & R50 	& 1000 \\
%               & R152    & 200\\
%               & R152    & 1000\\
%             \toprule
%         \end{tabular}
%         \caption{\small \emph{Accuracy} of student network (ResNet50) on ImageNet-1k distilled from teacher networks with different pre-training epochs.}
%         \label{tab:first_table}

% \end{minipage}
% \end{table}


% \begin{table}[!htb]
% \begin{minipage}{.42\linewidth}
%     \centering
%     % \medskip
%         % \setlength{\tabcolsep}{5.4pt}
%         % \small
%     \includegraphics[width=.99\textwidth]{images/distill_source.pdf}
%     \vspace{-6mm}
%     \caption{\small \emph{Accuracy} (\%) of student network on ImageNet distilling from \textit{wider} ResNet. }
%     \label{fig:wider}
% \end{minipage}\hfill
% \begin{minipage}{.56\linewidth}
%     \centering
%     \medskip
%     \setlength{\tabcolsep}{3.4pt}
%     \small
%     \begin{tabular}{cccccc}
%         \toprule
%         \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multirow{2}{*}{\textbf{Epochs}} & \multicolumn{1}{c}{\textbf{\textit{T}-Linear}} & \multicolumn{2}{c}{\textbf{\textit{S}-Linear}} \\
%         \cmidrule(lr){4-4}\cmidrule(lr){5-6}
%          &  & & Top-1 & Top-1 & Top-5\\
%         \midrule
%         \multirow{5}{*}{ResNet18} & MoCo& 200 & 60.6 \\
%           & MoCo-v2 & 200 & 67.7 \\
%           & MoCo-v2 & 800 & 71.1 \\
%           & SimCLR & 200 \\
%           & {\large S}WAV & 800 & 75.3 \\
%         \toprule
%     \end{tabular}
%     \caption{\small \emph{Accuracy} of student network on ImageNet distilling from variants of self-supervised ResNet-50. \textit{T/S}-Linear represents testing accuracy (\%) of Teacher and Student respectively. }
%     \label{tbl:variants}
% \end{minipage}
%     % \captionlistentry[table]{A table beside a figure}
%     % \captionsetup{labelformat=andtable}
%     % \caption{\small \emph{Accuracy} of student network on ImageNet distilling from \textit{wider} ResNet (left), and variants of self-supervised ResNet-50 (right). \textit{T/S}-Linear represents testing accuracy (\%) of Teacher and Student respectively. }
% \end{table}
% \usepackage[table, dvipsnames]{xcolor}

% \begin{table}[t]
% \vspace{-4mm}
% \begin{minipage}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=1\textwidth]{images/iclr_bar.pdf}
%         \captionof{figure}{\small \emph{Accuracy} (\%) of student networks (EfficientNet-b0 and ResNet-18) on ImageNet distilled from \textit{wider} MoCo-v2 pre-trained ResNet (ResNet-50/101/152{\scriptsize $\times$2)}. }
%         \label{fig:wider}
% \end{minipage}\hfill
% \begin{minipage}[b]{0.48\linewidth}
%     \centering
%     \medskip
%     \setlength{\tabcolsep}{3.2pt}
%     \caption{\small ImageNet-1k \emph{Accuracy} (\%) of student network (ResNet-18) distilled from variants of self-supervised ResNet-50. P-E/D-E represent the pre-training and distillation epochs. {T./S.}-Top represent testing accuracy of Teacher and Student. $^*$ represents distillation using additional small patches. First row is the ResNet-18 \textit{SSL} baseline using MoCo-v2 trained for 200 epochs.}
%     \small
%     \scalebox{0.9}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \textbf{Teacher} & \textbf{P-E} &  \textbf{D-E} & \textbf{T. Top-1} & \textbf{S. Top-1} & \textbf{S. Top-5} \\
%         \midrule
%         \xmark & \xmark & \xmark & \xmark & 52.5 & 77.0 \\
%         \hdashline \\[-1.9ex]
%         MoCo& 200 & 200 & 60.6 & 52.1 &77.0 \\
%         SimCLR & 200 & 200 & 65.6 &  57.5 & 81.7\\
%         MoCo-v2 & 200 & 200 & 67.4 & 57.6 & 81.8 \\
%         & 800 & 200 & 71.1 &60.5 & 83.5 \\
%         S{\small WAV}  & 800 & 100 & 75.3 &  61.1 & 83.8\\
%         & 800 & 200 & 75.3 &  61.7 & 84.2\\
%         & 800 & 400 & 75.3 & 62.0 &84.4 \\
%         SWAV$^*$  & 800 & 200 & 75.3 &  \cellcolor{cellcolor}\textbf{62.6} & \cellcolor{cellcolor}\textbf{84.8}\\
%         \toprule
%     \end{tabular}
%     }
%     \label{tbl:variants}
% \end{minipage}
% \end{table}

\begin{table}
	\begin{minipage}{0.48\linewidth}
    \centering
    \medskip
    \setlength{\tabcolsep}{3.2pt}
    \caption{\small ImageNet-1k \emph{Accuracy} (\%) of student network (ResNet-18) distilled from variants of self-supervised ResNet-50. P-E/D-E represent the pre-training and distillation epochs. {T./S.}-Top represent testing accuracy of Teacher and Student. $^*$ represents distillation using additional small patches. First row is the ResNet-18 \textit{SSL} baseline using MoCo-v2 trained for 200 epochs.}
    \vspace{-2mm}
    \small
    \scalebox{0.9}{
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Teacher} & \textbf{P-E} &  \textbf{D-E} & \textbf{T. Top-1} & \textbf{S. Top-1} & \textbf{S. Top-5} \\
        \midrule
        \xmark & \xmark & \xmark & \xmark & 52.5 & 77.0 \\
        \hdashline \\[-1.9ex]
        MoCo& 200 & 200 & 60.6 & 52.1 &77.0 \\
        SimCLR & 200 & 200 & 65.6 &  57.5 & 81.7\\
        MoCo-v2 & 200 & 200 & 67.4 & 57.9 & 82.0 \\
        & 800 & 200 & 71.1 &60.5 & 83.5 \\
        S{\small WAV}  & 800 & 100 & 75.3 &  61.1 & 83.8\\
        & 800 & 200 & 75.3 &  61.7 & 84.2\\
        & 800 & 400 & 75.3 & 62.0 &84.4 \\
        SWAV$^*$  & 800 & 200 & 75.3 &  \cellcolor{cellcolor}\textbf{62.6} & \cellcolor{cellcolor}\textbf{84.8}\\
        \toprule
    \end{tabular}
    }
    \label{tbl:variants}
	\end{minipage}\hfill
	\begin{minipage}{0.46\linewidth}
        \centering
        \vspace{4mm}
        \includegraphics[width=1\textwidth]{images/iclr_bar.pdf}
        \captionof{figure}{\small \emph{Accuracy} (\%) of student networks (EfficientNet-b0 and ResNet-18) on ImageNet distilled from \textit{wider} MoCo-v2 pre-trained ResNet (ResNet-50/101/152{\scriptsize $\times$2)}. }
        \vspace{-3mm}
        \label{fig:wider}
	\end{minipage}
\end{table}

==> ICLR20_Distillatio (2)/tables/distill_loss.tex <==

\begin{table}[t]
\begin{minipage}{.46\linewidth}
{\normalsize
    \centering
    \medskip
    \setlength{\tabcolsep}{1.1pt}
    \caption{\small  Top-1/5 accuracy of linear classification results on ImageNet using different distillation strategies on ResNet-18 (student) and ResNet-50 (teacher) architectures.}
    \vspace{-3mm}
    \begin{tabular}{ccc}
        \toprule
        \textbf{Method} &  Top-1 Acc. & Top-5 Acc.\\
        \midrule
        \emph{l2-Distance} & 55.3 & 80.3  \\
        \textit{K}-Means & 51.0 & 75.8 \\
        Online Clustering & 56.4 & 81.2  \\
        Binary Contr. Loss &  57.4 & 81.5  \\
        {\large S}EED + MoCo-V2 & 57.6& 81.8  \\
        {\large S}EED & \cellcolor{cellcolor}\textbf{57.9 }& \cellcolor{cellcolor}\textbf{82.0}  \\
        \toprule
    \end{tabular}
    \label{tbl:loss}
    }
\end{minipage}\hfill
\begin{minipage}{.5\linewidth}
{\normalsize
    \centering
    \medskip
    \setlength{\tabcolsep}{3.4pt}
    \caption{\small Effect of $\tau^T$ for the distillation of ResNet-18 (student), ResNet-50 (teacher) on multiple datasets. }
    \vspace{-2mm}
    \begin{tabular}{cccccc}
       \toprule
       \multirow{2}{*}{ \textbf{$\tau^{T}$}}&  \multicolumn{2}{c}{\textbf{ImageNet}}&  \multicolumn{1}{c}{\textbf{CIFAR-10}} & \multicolumn{1}{c}{\textbf{CIFAR-100}} \\
       \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} 
       & Top-1  & Top-5 & Top-1 & Top-1 \\
        \midrule
        0.3 &  54.8 &80.0 & 78.7 & 46.6\\
        % 0.2 &  &  & & & 78.6\\
        0.1 & 54.9 & 80.1 & 83.0 & 50.1\\
        0.05 & 56.5 & 81.3 & 84.4 & 56.2  \\
        0.01 & \cellcolor{cellcolor}\textbf{57.9} & \cellcolor{cellcolor}\textbf{82.0} & \cellcolor{cellcolor}\textbf{87.5} & 60.6 \\
        1e-3 & 57.6 & 81.8 & 86.9 & \cellcolor{cellcolor}\textbf{60.8}  \\
        \toprule
    \end{tabular}
    \label{tbl:negtive}
}
\end{minipage}
\end{table}

==> ICLR20_Distillatio (2)/tables/semi_imagenet.tex <==

\begin{table}[t]
% \vspace{-3mm}
%   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

\setlength{\tabcolsep}{4.8pt}
\begin{center}
\renewcommand{\arraystretch}{1.07} % Default value: 1
{
\small
\scalebox{0.94}{
\begin{tabular}{cccccccccccccccc} 
\toprule
\\[-2.8ex]
\multirow{2}{*}{\backslashbox{\textbf{T}}{\textbf{S}}} &   \multicolumn{3}{c}{\textbf{Eff-b0}} & \multicolumn{3}{c}{\textbf{Mob-v3}} & \multicolumn{3}{c}{\textbf{R-18}} & \multicolumn{3}{c}{\textbf{R-34}} & \multicolumn{3}{c}{\textbf{R-50}}  \\
 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\\[-2.8ex]
\hline \\[-2.ex]
%  \xmark & & 39.1 & 64.6 & 27.5 & 36.3 & 62.2 & 36.7 & 52.5 & 77.0 & 41.5 & 57.4 & 81.6 & 46.1 & 67.4 & 87.8 \\ \hdashline [.8ex]
 \xmark & & 39.1 & 64.6 & 27.5 & 36.3 & 62.2 & 36.7 & 52.5 & 77.0 & 41.5 & 57.4 & 81.6 & 46.1 & 67.4 & 87.8 \\[.2ex] \hdashline \\[-1.9ex]
 \multirow{1}{*}{R-50} & 46.0 & 61.3 & 82.7 & 44.8 & 55.2 & 80.3 & 43.4 & 57.6 & 81.8 & 45.2 & 58.5 & 82.6 & 46.1 & 67.5 & 87.8 \\[-.8ex]
 {\tiny $\Delta$}& & {\tiny $\mathcolor{darkgreen}{\textbf{+22.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+18.1}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+17.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.9}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+5.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+4.8}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+3.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+1.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+1.0}}$} &	{\tiny \textbf{+0.0}} & 	{\tiny \textbf{+0.1}} & 	{\tiny \textbf{+0.0}}
\\[.2ex] \hdashline \\[-1.9ex]
  \multirow{1}{*}{R-101} & 50.1 & 63.0 & 83.8 & 48.8 & 59.9 & 83.5 & 48.6 & 58.9 & 82.5 & 50.5 & 61.6 & 84.9 & 52.3 & 69.1 & 88.7 \\[-.8ex]
 {\tiny $\Delta$} & & {\tiny $\mathcolor{darkgreen}{\textbf{+23.9}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+19.2}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+21 .3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+23.6}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+21.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+11.9}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.4}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+5.5}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+9.0}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+4.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+3.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+6.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+1.7}}$} &	{\tiny $	{\tiny \textbf{+0.9}} $}
 \\[.2ex] \hdashline \\[-1.9ex]
  \multirow{1}{*}{R-152}& 50.7 & 65.3 & 86.0 & 49.5 & 61.4 & 84.6 & 49.1 & 59.5 & 83.3 & 51.4 & 62.7 & 85.8 & 53.2 & 70.4 & 90.5 \\[-.8ex]
 {\tiny $\Delta$} & & {\tiny$\mathcolor{darkgreen}{\textbf{+26.2}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+21.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+22.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+25.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+22.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+12.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+7.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+6.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+9.9}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+5.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+4.2}}$} & 	{\tiny$\mathcolor{darkgreen}{\textbf{+7.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+3.0}}$}	& {\tiny$\mathcolor{darkgreen}{\textbf{+2.7}}$}
 \\[.2ex] \hdashline \\[-1.9ex]
  \multirow{1}{*}{R50{\tiny $\times$2}^{*}} & & & & & & & & & & & & & 54.0 & 74.3 & 92.2  \\[-.8ex]
 {\tiny $\Delta$} & \\

\toprule
\end{tabular}
}
}
\caption{
{\small
Top-1 accuracy for semi-supervised evaluations using 1\% and 10\% label fractions. 
}}
\label{tbl:imgnet}
\end{center}
\vspace{-8mm}
\end{table}

==> ICLR20_Distillatio (2)/tables/transfer.tex <==

% \begin{table}[ht]


% \setlength{\tabcolsep}{2.5pt}
% \small
% {
% \begin{center}
% % \renewcommand{\arraystretch}{1} % Default value: 1
%     \begin{tabular}{ccccccccccccc}
%     \cmidrule[\heavyrulewidth]{1-13}
%     {\small \textbf{Method}} & {\scriptsize Food101} & {\scriptsize CIFAR10} & {\scriptsize CIFAR100} & {\scriptsize Birdsnap} & {\scriptsize SUN397}  & {\scriptsize Cars} & {\scriptsize Aircraft} & {\scriptsize VOC2007} & {\scriptsize DTD} & {\scriptsize Pets} & {\scriptsize Caltech-101} & {\scriptsize Flowers} \\
%     \midrule
%     % \multicolumn{13}{l}{\emph{Linear evaluation:}}\\
%     % \midrule
%     % \simclr (repro)&$72.8$&$90.5$&$74.4$&$42.4$&$60.6$&$49.3$& $49.8$ & $81.4$&$\bf{75.7}$&$84.6$&$89.3$&$92.6$
%     Supervised & $72.3$ & $93.6$ & $78.3$ &$53.7$ & $61.9$ & $66.7$ &$ 61.0$ & $82.8$ & $74.9$ & $91.5$ & $94.5$ & $94.7 $\\
%     SimCLR & $68.4$ & $90.6$ & $71.6$ &$37.4$ & $58.8$ & $50.3$ &$ 50.3$ & $80.5$ & $74.5$ & $83.6$ & $90.3$ & $91.2 $\\
%     CMC$^*$ \\
%     MoCo$^*$ &  \\
%     MoCo-v2$^*$ \\
%     BYOL & {75.3} & 91.3 & {78.4}& {57.2}& {62.2}& {67.8}& 60.6 & 82.5& 75.5 & 90.4 & 94.2 & {96.1} \\
%     \\[-2ex]
%      \hdashline \\[-2ex]
%     Ours \\
%     % \midrule
%     % \multicolumn{13}{l}{\emph{Fine-tuned:}}\\
%     % \midrule
%     % \algo (ours) &\cellcolor{pearDark!20}$\bf{88.5}$&\cellcolor{pearDark!20}$\bf{97.8}$&\cellcolor{pearDark!20}$86.1$&\cellcolor{pearDark!20}$\bf{76.3}$&\cellcolor{pearDark!20}$63.7$&\cellcolor{pearDark!20}$91.6$&\cellcolor{pearDark!20}$\bf{88.1}$&\cellcolor{pearDark!20} $\bf{85.4}$ &\cellcolor{pearDark!20}$\bf{76.2}$&\cellcolor{pearDark!20}$91.7$&\cellcolor{pearDark!20}$\bf{93.8}$&\cellcolor{pearDark!20}$97.0$\\
%     % \simclr (repro) & $87.5$ & $97.4$ & $85.3$ & $75.0$ & $63.9$ & $91.4$ & $87.6$ & $84.5$ & $75.4$ & $89.4$ & $91.7$ & $96.6$  \\
%     % \simclr \cite{SimCLR}  & $88.2$ & $97.7$ & $85.9$ & $75.9$ & $63.5$ & $91.3$ & $88.1$ & $84.1$ & $73.2$ & $89.2$ & $92.1$ & $97.0$  \\
%     % \supervisedbaseline~\cite{SimCLR} & $88.3$ & $97.5$ & $\bf{86.4}$ & $75.8$ & $\bf{64.3}$ & $\bf{92.1}$ & $86.0$ & $85.0$ & $74.6$ & $\bf{92.1}$ & $93.3$ & $\bf{97.6}$ \\
%     % Random init \cite{SimCLR} & $86.9$ & $95.9$ & $80.2$ & $76.1$  & $53.6$ & $91.4$ & $85.9$ & $67.3$ & $64.8$ & $81.5$ & $72.6$ & $92.0$  \\
%     \bottomrule
%     \end{tabular}
%     \caption{
%         {
%         Feature transferability on different domains. Linear classification results finetuned on the representations from on ImageNet with the standard ResNet-50 architecture.
%         }}
% \label{tbl:transfer}
% \end{center}
% }
% \end{table}


==> ICLR20_Distillatio (2)/tables/voc_det.tex <==
% \begin{table}[t]

% %   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

% \setlength{\tabcolsep}{3pt}
% \begin{center}
% \renewcommand{\arraystretch}{1.2} % Default value: 1
% \begin{tabular}{ccccc}
% \toprule
% \\[-3.5ex]
% \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multicolumn{3}{c}{\textbf{VOC07 Detection}} \\
% \cmidrule(lr){3-5}\\[-3.5ex]
%  &  & AP^{\text{bb}}  & AP^\text{bb}_{50}  & AP^\text{bb}_{75} \\
%  \\[-3.5ex]
% \midrule
% RetNet18 & \xmark 	& 46.1 & 74.5 & 48.6 \\
% ResNet34 & \xmark 	& 53.6 & 79.1 & 58.7   \\
% ResNet50 & \xmark 	& 57.0 & 82.4 & 63.6 \\
% % ResNet101 & \xmark 	& \\
% % ResNet152 & \xmark 	 \\
%  \hdashline \\[-3ex]
 
% \multirow{3}{*}{{RetNet18}} & ResNet50 	& 46.1 {\scriptsize ( 0.0)} & 74.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 49.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & ResNet101 	& 46.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 75.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+1.3})}$} & 49.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} \\
%  & ResNet152 	& \\
% \hdashline \\[-3ex]

% \multirow{3}{*}{{ResNet34}} & ResNet50 	& 53.7  {\scriptsize (+0.1)}& 79.4 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$}  & 59.2 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & ResNet101 	&  54.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$} & 79.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 59.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$}\\
%  & ResNet152 	& \\
% \hdashline \\[-3ex]

% \multirow{3}{*}{{ResNet50}} & ResNet50 	& \\
%  & ResNet101 	&  57.1 {\scriptsize (+0.1)} & 82.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 63.8  {\scriptsize (+0.2)}\\
%  & ResNet152 	& \\


% \toprule
% \end{tabular}
% \caption{
% {\small
% Object detection and instance segmentation fine-tuned on VOC07 and COCO: bounding-box AP (AP$^{bb}$) and mask AP (AP$^{mk}$) evaluated
% on VOC07-val and COCO-val2017 respectively. The first several rows show the baselines from unsupervised backbones without distillation. R* represents the ResNet\{18, 32, 50\} architectures.
% }}
% \label{tbl:cifar100_diff}
% \end{center}
% \vspace{-10pt}
% \end{table}

\begin{table}[t]
\vspace{-4mm}
%   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

\setlength{\tabcolsep}{2.2pt}
\begin{center}
\renewcommand{\arraystretch}{1.2} % Default value: 1
\caption{
{\small
Object detection and instance segmentation results using contrastive self-supervised learning and {\large S}EED distillation using ResNet-18 as backbone: bounding-box AP (AP$^{bb}$) and mask AP (AP$^{mk}$) evaluated
on VOC07-val and COCO testing split. More results on different backbones can be found in the Appendix. Subscript in green represents improvement is larger than 0.3.
}}
% \vspace{-2mm}
{\small
\begin{tabular}{ccccccccccc}
\toprule
\\[-3.5ex]
\multirow{2}{*}{\textbf{S}} &  \multirow{2}{*}{\textbf{T}} &  \multicolumn{3}{c}{\textbf{VOC Obj. Det.}} &  \multicolumn{3}{c}{\textbf{COCO Obj. Det.}} & \multicolumn{3}{c}{\textbf{COCO Inst. Segm.}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}\\[-3.5ex]
 &  & AP$^{\text{bb}}$  & AP$^\text{bb}_{50}$  & AP$^\text{bb}_{75}$ & AP$^{\text{bb}}$  & AP$^\text{bb}_{50}$  & AP$^\text{bb}_{75}$ & AP$^{\text{mk}}$  & AP$^\text{mk}_{50}$  & AP$^\text{mk}_{75}$ \\
 \\[-3.5ex]
\midrule


% ResNet101 & \xmark 	& \\
% ResNet152 & \xmark 	 \\
%  \hdashline \\[-3ex]
 
\multirow{5}{*}{{\textbf{R-18}}}  & \xmark 	& 46.1 & 74.5 & 48.6 & 35.0  &  53.9 & 37.7 & 31.0 & 51.1 & 33.1\\
& \textbf{R-50} 	& 46.1{\scriptsize ( 0.0)} & 74.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 49.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$} & 35.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 54.2{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 37.8{\scriptsize (+0.1)} & 31.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.1})}$} & 51.1{\scriptsize ( 0.0)} & 33.2{\scriptsize (+0.1)} \\
 & \textbf{R-101} 	& 46.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 75.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+1.3})}$} & 49.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 35.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 54.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 37.9{\scriptsize (+0.2)} & 31.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 51.3{\scriptsize (+0.2)} & 33.4{\scriptsize (+0.3)}\\
 & \textbf{R-152} 	&  46.8{\scriptsize$\mathcolor{darkgreen}{(\textbf{+0.7})}$}  & 75.9{\scriptsize$\mathcolor{darkgreen}{(\textbf{+1.4})}$}  & 50.2{\scriptsize$\mathcolor{darkgreen}{(\textbf{+1.6})}$}  & 35.4{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 54.4{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$} & 38.0{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 31.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 51.4{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 33.4{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} \\
%  & \multirow{1}{*}{\textbf{R-50{\tiny $\times$2}}} & 1835 & & & 1836\\
% \hdashline \\[-3ex]

% \multirow{4}{*}{{ResNet34}}  & \xmark 	& 53.6 & 79.1 & 58.7   \\
% & ResNet50 	& 53.7  {\scriptsize (+0.1)}& 79.4 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$}  & 59.2 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & ResNet101 	&  54.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$} & 79.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 59.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$}\\
%  & ResNet152 	& \\
% \hdashline \\[-3ex]

% \multirow{4}{*}{{ResNet50}}  & \xmark 	& 57.0 & 82.4 & 63.6 \\
% & ResNet50 	& \\
%  & ResNet101 	&  57.1 {\scriptsize (+0.1)} & 82.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 63.8  {\scriptsize (+0.2)}\\
%  & ResNet152 	& \\
\toprule
\end{tabular}
}
\label{tbl:voc}
\end{center}
% \vspace{-4mm}
\end{table}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> method.tex <==
\section{Method}


==> tables/coco_det_seg.tex <==
% \begin{table}[t]

% %   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

% \setlength{\tabcolsep}{3pt}
% \begin{center}
% \renewcommand{\arraystretch}{1.2} % Default value: 1
% \begin{tabular}{ccccccccccc}
% \toprule
% \\[-3.5ex]
% \multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} &  \multicolumn{3}{c}{\textbf{VOC07 Detection}} & \multicolumn{3}{c}{\textbf{COCO Detection}} & \multicolumn{3}{c}{\textbf{COCO Inst. Segment.}} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8} \cmidrule(lr){9-11}\\[-3.5ex]
%  &  & AP^{\text{bb}}  & AP^\text{bb}_{50}  & AP^\text{bb}_{75} & AP^{\text{bb}}  & AP^\text{bb}_{50}  & AP^\text{bb}_{75} & AP^{\text{mk}}  & AP^\text{mk}_{50}  & AP^\text{mk}_{75}\\
%  \\[-3.5ex]
% \midrule
% R18 & \xmark 	& 46.1 & 74.5 & 48.6 & 32.2 & 50.7 & 34.2 & 28.9 & 48.0 & 30.5 \\
% R34 & \xmark 	& 53.6 & 79.1 & 58.7 &  & &  \\
% R50 & \xmark 	& 57.0 & 82.4 & 63.6 & 35.6 & 57.3 & 37.6 & 40.7 & 60.5 & 44.1\\
% % ResNet101 & \xmark 	& \\
% % ResNet152 & \xmark 	 \\
%  \hdashline \\[-3ex]
 
% \multirow{3}{*}{{R18}} & R50 	& 46.1 {\scriptsize ( 0.0)} & 74.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$} & 49.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & R101 	& 46.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 75.8{\scriptsize $\mathcolor{darkgreen}{(\textbf{+1.3})}$} & 49.3{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 32.4{\scriptsize (+0.2)} & 51.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 34.5{\scriptsize (+0.3)} & 29.1{\scriptsize (+0.2)}&  48.2{\scriptsize (+0.2)} &  30.5{\scriptsize ( 0.0)}\\
%  & R152 	& \\
% \hdashline \\[-3ex]

% \multirow{3}{*}{{R34}} & R50 	& 53.7  {\scriptsize (+0.1)}& 79.4 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.3})}$}  & 59.2 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$}\\
%  & R101 	&  54.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.5})}$} & 79.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.7})}$} & 59.1 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$}\\
%  & R152 	& \\
% \hdashline \\[-3ex]

% \multirow{3}{*}{{R50}} & R50 	& \\
%  & R101 	&  57.1 {\scriptsize (+0.1)} & 82.8 {\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 63.8  {\scriptsize (+0.2)}\\
%  & R152 	& \\


% \toprule
% \end{tabular}
% \caption{
% {\small
% Object detection and instance segmentation fine-tuned on VOC07 and COCO: bounding-box AP (AP$^{bb}$) and mask AP (AP$^{mk}$) evaluated
% on VOC07-val and COCO-val2017 respectively. The first several rows show the baselines from unsupervised backbones without distillation. R* represents the ResNet\{18, 32, 50\} architectures.
% }}
% \label{tbl:cifar100_diff}
% \end{center}
% \vspace{-10pt}
% \end{table}

\begin{table}[t]
\setlength{\tabcolsep}{6pt}
\begin{center}
\renewcommand{\arraystretch}{1.2} % Default value: 1
{\small
\begin{tabular}{ccccccccccc}
\toprule
\\[-3.5ex]
\multirow{2}{*}{\textbf{Student}} &  \multirow{2}{*}{\textbf{Teacher}} & \multicolumn{3}{c}{\textbf{Object Detection}} & \multicolumn{3}{c}{\textbf{Instance Segmentation}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8} \cmidrule(lr){9-11}\\[-3.5ex]
 &  & AP$^{\text{bb}}$  & AP$^\text{bb}_{50}$  & AP$^\text{bb}_{75}$ & AP$^{\text{mk}}$  & AP$^\text{mk}_{50}$  & AP$^\text{mk}_{75}$\\
 \\[-3.5ex]
\midrule
ResNet18 & \xmark  & 32.2 & 50.7 & 34.2 & 28.9 & 48.0 & 30.5 \\
ResNet34 & \xmark  &  & &  \\
ResNet50 & \xmark  & 35.6 & 57.3 & 37.6 & 40.7 & 60.5 & 44.1\\
% ResNet101 & \xmark 	& \\
% ResNet152 & \xmark 	 \\
 \hdashline \\[-3ex]
 
\multirow{3}{*}{{ResNet18}} & ResNet50 \\
 & ResNet101 	& 32.4{\scriptsize (+0.2)} & 51.1{\scriptsize $\mathcolor{darkgreen}{(\textbf{+0.4})}$} & 34.5{\scriptsize (+0.3)} & 29.1{\scriptsize (+0.2)}&  48.2{\scriptsize (+0.2)} &  30.5{\scriptsize ( 0.0)}\\
 & ResNet152 	& \\
\hdashline \\[-3ex]

\multirow{3}{*}{{ResNet34}} & ResNet50 \\
 & ResNet101 	& \\
 & ResNet152 	& \\
\hdashline \\[-3ex]

\multirow{3}{*}{{ResNet50}} & ResNet50 	& \\
 & ResNet101 	& \\
 & ResNet152 	& \\
\toprule
\end{tabular}
}
\caption{
{\small
Object detection and instance segmentation fine-tuned on COCO: bounding-box AP (AP$^{bb}$) and mask AP (AP$^{mk}$) evaluated
on VOC07-val and COCO-val2017 respectively. The first several rows show the baselines from unsupervised backbones without distillation. 
}}
\label{tbl:cifar100_diff}
\end{center}
\vspace{-10pt}
\end{table}


==> tables/semi_imagenet.tex <==

\begin{table}[t]
% \vspace{-3mm}
%   \begin{tabular}{@{\extracolsep{4pt}}rrrrrrrrr@{}}

\setlength{\tabcolsep}{4.8pt}
\begin{center}
\renewcommand{\arraystretch}{1.07} % Default value: 1
{
\small
\scalebox{0.94}{
\begin{tabular}{cccccccccccccccc} 
\toprule
\\[-2.8ex]
\multirow{2}{*}{\backslashbox{\textbf{T}}{\textbf{S}}} &   \multicolumn{3}{c}{\textbf{Eff-b0}} & \multicolumn{3}{c}{\textbf{Mob-v3}} & \multicolumn{3}{c}{\textbf{R-18}} & \multicolumn{3}{c}{\textbf{R-34}} & \multicolumn{3}{c}{\textbf{R-50}}  \\
 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 & \textit{K} & T-1 & T-5 \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\\[-2.8ex]
\hline \\[-2.ex]
%  \xmark & & 39.1 & 64.6 & 27.5 & 36.3 & 62.2 & 36.7 & 52.5 & 77.0 & 41.5 & 57.4 & 81.6 & 46.1 & 67.4 & 87.8 \\ \hdashline [.8ex]
 \xmark & & 39.1 & 64.6 & 27.5 & 36.3 & 62.2 & 36.7 & 52.5 & 77.0 & 41.5 & 57.4 & 81.6 & 46.1 & 67.4 & 87.8 \\[.2ex] \hdashline \\[-1.9ex]
 \multirow{1}{*}{R-50} & 46.0 & 61.3 & 82.7 & 44.8 & 55.2 & 80.3 & 43.4 & 57.6 & 81.8 & 45.2 & 58.5 & 82.6 & 46.1 & 67.5 & 87.8 \\[-.8ex]
 {\tiny $\Delta$}& & {\tiny $\mathcolor{darkgreen}{\textbf{+22.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+18.1}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+17.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.9}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+18.1}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+5.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+4.8}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+3.7}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+1.1}}$} & 	{\tiny $\mathcolor{darkgreen}{\textbf{+1.0}}$} &	{\tiny \textbf{+0.0}} & 	{\tiny \textbf{+0.1}} & 	{\tiny \textbf{+0.0}}
\\[.2ex] \hdashline \\[-1.9ex]
  \multirow{1}{*}{R-101} & 50.1 & 63.0 & 83.8 & 48.8 & 59.9 & 83.5 & 48.6 & 58.9 & 82.5 & 50.5 & 61.6 & 84.9 & 52.3 & 69.1 & 88.7 \\[-.8ex]
 {\tiny $\Delta$} & & {\tiny $\mathcolor{darkgreen}{\textbf{+23.9}}$}	& {\tiny $\mathcolor{darkgreen}{\textbf{+19.2}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+21 .3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+23.6}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+21.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+11.9}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+6.4}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+5.5}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+9.0}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+4.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+3.3}}$} &	{\tiny $\mathcolor{darkgreen}{\textbf{+6.2}}$} & {\tiny $\mathcolor{darkgreen}{\textbf{+1.7}}$} &	{\tiny $	{\tiny \textbf{+0.9}} $}
 \\[.2ex] \hdashline \\[-1.9ex]
  \multirow{1}{*}{R-152}& 50.7 & 65.3 & 86.0 & 49.5 & 61.4 & 84.6 & 49.1 & 59.5 & 83.3 & 51.4 & 62.7 & 85.8 & 53.2 & 70.4 & 90.5 \\[-.8ex]
 {\tiny $\Delta$} & & {\tiny$\mathcolor{darkgreen}{\textbf{+26.2}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+21.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+22.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+25.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+22.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+12.4}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+7.0}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+6.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+9.9}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+5.3}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+4.2}}$} & 	{\tiny$\mathcolor{darkgreen}{\textbf{+7.1}}$} &	{\tiny$\mathcolor{darkgreen}{\textbf{+3.0}}$}	& {\tiny$\mathcolor{darkgreen}{\textbf{+2.7}}$}
 \\[.2ex] \hdashline \\[-1.9ex]
  \multirow{1}{*}{R50{\tiny $\times$2}^{*}} & & & & & & & & & & & & & 54.0 & 74.3 & 92.2  \\[-.8ex]
 {\tiny $\Delta$} & \\

\toprule
\end{tabular}
}
}
\caption{
{\small
Top-1 accuracy for semi-supervised evaluations using 1\% and 10\% label fractions. 
}}
\label{tbl:imgnet}
\end{center}
\vspace{-8mm}
\end{table}

==> tables/transfer.tex <==

% \begin{table}[ht]


% \setlength{\tabcolsep}{2.5pt}
% \small
% {
% \begin{center}
% % \renewcommand{\arraystretch}{1} % Default value: 1
%     \begin{tabular}{ccccccccccccc}
%     \cmidrule[\heavyrulewidth]{1-13}
%     {\small \textbf{Method}} & {\scriptsize Food101} & {\scriptsize CIFAR10} & {\scriptsize CIFAR100} & {\scriptsize Birdsnap} & {\scriptsize SUN397}  & {\scriptsize Cars} & {\scriptsize Aircraft} & {\scriptsize VOC2007} & {\scriptsize DTD} & {\scriptsize Pets} & {\scriptsize Caltech-101} & {\scriptsize Flowers} \\
%     \midrule
%     % \multicolumn{13}{l}{\emph{Linear evaluation:}}\\
%     % \midrule
%     % \simclr (repro)&$72.8$&$90.5$&$74.4$&$42.4$&$60.6$&$49.3$& $49.8$ & $81.4$&$\bf{75.7}$&$84.6$&$89.3$&$92.6$
%     Supervised & $72.3$ & $93.6$ & $78.3$ &$53.7$ & $61.9$ & $66.7$ &$ 61.0$ & $82.8$ & $74.9$ & $91.5$ & $94.5$ & $94.7 $\\
%     SimCLR & $68.4$ & $90.6$ & $71.6$ &$37.4$ & $58.8$ & $50.3$ &$ 50.3$ & $80.5$ & $74.5$ & $83.6$ & $90.3$ & $91.2 $\\
%     CMC$^*$ \\
%     MoCo$^*$ &  \\
%     MoCo-v2$^*$ \\
%     BYOL & {75.3} & 91.3 & {78.4}& {57.2}& {62.2}& {67.8}& 60.6 & 82.5& 75.5 & 90.4 & 94.2 & {96.1} \\
%     \\[-2ex]
%      \hdashline \\[-2ex]
%     Ours \\
%     % \midrule
%     % \multicolumn{13}{l}{\emph{Fine-tuned:}}\\
%     % \midrule
%     % \algo (ours) &\cellcolor{pearDark!20}$\bf{88.5}$&\cellcolor{pearDark!20}$\bf{97.8}$&\cellcolor{pearDark!20}$86.1$&\cellcolor{pearDark!20}$\bf{76.3}$&\cellcolor{pearDark!20}$63.7$&\cellcolor{pearDark!20}$91.6$&\cellcolor{pearDark!20}$\bf{88.1}$&\cellcolor{pearDark!20} $\bf{85.4}$ &\cellcolor{pearDark!20}$\bf{76.2}$&\cellcolor{pearDark!20}$91.7$&\cellcolor{pearDark!20}$\bf{93.8}$&\cellcolor{pearDark!20}$97.0$\\
%     % \simclr (repro) & $87.5$ & $97.4$ & $85.3$ & $75.0$ & $63.9$ & $91.4$ & $87.6$ & $84.5$ & $75.4$ & $89.4$ & $91.7$ & $96.6$  \\
%     % \simclr \cite{SimCLR}  & $88.2$ & $97.7$ & $85.9$ & $75.9$ & $63.5$ & $91.3$ & $88.1$ & $84.1$ & $73.2$ & $89.2$ & $92.1$ & $97.0$  \\
%     % \supervisedbaseline~\cite{SimCLR} & $88.3$ & $97.5$ & $\bf{86.4}$ & $75.8$ & $\bf{64.3}$ & $\bf{92.1}$ & $86.0$ & $85.0$ & $74.6$ & $\bf{92.1}$ & $93.3$ & $\bf{97.6}$ \\
%     % Random init \cite{SimCLR} & $86.9$ & $95.9$ & $80.2$ & $76.1$  & $53.6$ & $91.4$ & $85.9$ & $67.3$ & $64.8$ & $81.5$ & $72.6$ & $92.0$  \\
%     \bottomrule
%     \end{tabular}
%     \caption{
%         {
%         Feature transferability on different domains. Linear classification results finetuned on the representations from on ImageNet with the standard ResNet-50 architecture.
%         }}
% \label{tbl:transfer}
% \end{center}
% }
% \end{table}

